Learning to Generalize from Sparse and Underspecified Rewards

We consider the problem of learning from sparse and underspecified rewards, where an agent receives a complex input, such as a natural language instruction, and needs to generate a complex response, such as an action sequence, while only receiving binary success-failure feedback. Such success-failure rewards are often underspecified: they do not distinguish between purposeful and accidental success. Generalization from underspecified rewards hinges on discounting spurious trajectories that attain accidental success, while learning from sparse feedback requires effective exploration. We address exploration by using a mode covering direction of KL divergence to collect a diverse set of successful trajectories, followed by a mode seeking KL divergence to train a robust policy. We propose Meta Reward Learning (MeRL) to construct an auxiliary reward function that provides more refined feedback for learning. The parameters of the auxiliary reward function are optimized with respect to the validation performance of a trained policy. The MeRL approach outperforms our alternative reward learning technique based on Bayesian Optimization, and achieves the state-of-the-art on weakly-supervised semantic parsing. It improves previous work by 1.2% and 2.4% on WikiTableQuestions and WikiSQL datasets respectively.

==> details.tex <==
We present some implementation details of our method on
weakly-supervised semantic parsing here. We will release the source
code upon public release of the paper.

{\bf Experiment Setup.} Our implementation is based on the open
source implementation of MAPO~\cite{NIPS2018_8204} in
Tensorflow~\cite{abadi2016tensorflow}.  We use the same model
architecture as MAPO which combines a seq2seq model augmented by a
key-variable memory~\cite{liang2017nsm} with a domain specific
language interpreter. We utilized the hyperparameter tuning
service~\cite{golovin2017google} provided by Google Cloud for our
Bayesian Optimization approach (BoRL).

{\bf Auxiliary Reward Features.}
In our semantic parsing experiments, we used the same preprocessing as implemented in MAPO.
The natural language queries are preprocessed to identify numbers and date-time entities. In addition,
phrases in the query that appear in the table entries are converted to string entities and the columns
in the table that have a phrase match are assigned a column feature weight based on the match.

We used the following features for our auxiliary reward for both \textsc{WikiTableQuestions} and \textsc{WikiSQL}:
\begin{itemize}
	\itemsep-0.5em
	\item $\vf_1$: Fraction of total entities in the program weighted by the entity length
	\item $\vf_2$, $\vf_3$, $\vf_4$: Fraction of date-time, string and number entities in the program weighted by the entity length respectively
	\item $\vf_5$: Fraction of total entities in the program
	\item $\vf_6$: Fraction of longest entities in the program
	\item $\vf_7$: Fraction of columns in the program weighted by the column weight
	\item $\vf_8$: Fraction of total columns in the program with non-zero column weight
	\item $\vf_9$: Fraction of columns used in the program with the highest column column weight
	\item $\vf_{10}$: Fractional number of expressions in the program
	\item $\vf_{11}$: Sum of entities and columns weighted by their length and column weight respectively divided by the number of expressions in the program
\end{itemize}




==> fig3.tex <==
% \small
% \begin{tabular}{@{}l@{\hspace*{.1cm}}l@{}}
% \\
% \end{tabular}

